Shape Optimization for the Mitigation of Coastal Erosion via Porous Shallow Water Equations

Coastal erosion describes the displacement of land caused by destructive sea waves, currents or tides. Major efforts have been made to mitigate these effects using groynes, breakwaters and various other structures. We address this problem by applying shape optimization techniques on the obstacles. We model the propagation of waves towards the coastline using two-dimensional porous Shallow Water Equations with artificial viscosity. The obstacle's shape, which is assumed to be permeable, is optimized over an appropriate cost function to minimize the height and velocities of water waves along the shore, without relying on a finite-dimensional design space, but based on shape calculus.

==> objective_mentawai_3.tex <==
%auto-ignore
% This file was created with tikzplotlib v0.9.13.
\begin{tikzpicture}

\begin{axis}[
legend cell align={left},
legend style={fill opacity=0.8, draw opacity=1, text opacity=1, draw=white!80!black},
tick align=outside,
tick pos=left,
title={Objective Value},
x grid style={white!69.0196078431373!black},
xlabel={Iteration},
xmajorgrids,
xmin=-2.85, xmax=59.85,
xtick style={color=black},
y grid style={white!69.0196078431373!black},
ylabel={Objective},
ymajorgrids,
ymin=12.9048466810822, ymax=13.377530067043,
ytick style={color=black}
]
\addplot [line width=1.64pt, blue]
table {%
0 13.3560444585903
1 13.341946161729
2 13.3280126126204
3 13.3142544812002
4 13.3006819239138
5 13.2873049230834
6 13.2741332877345
7 13.2611764351312
8 13.2484430433787
9 13.2359407583737
10 13.2236759925069
11 13.2116538215457
12 13.1998779991203
13 13.1883510084715
14 13.1770741782146
15 13.1660478220088
16 13.1552713718793
17 13.1447435347261
18 13.1344624278309
19 13.1244257762013
20 13.1146310792695
21 13.1050757409714
22 13.0957572170168
23 13.0866731207977
24 13.0778212867108
25 13.0691998804387
26 13.0608073593218
27 13.0526425121673
28 13.0447044686946
29 13.0369927058578
30 13.0295071172858
31 13.0222480403512
32 13.0152163215996
33 13.0084133651965
34 13.0018411910805
35 12.9955024577075
36 12.9894005018418
37 12.9835393834412
38 12.977923817691
39 12.9725591759405
40 12.9674514385986
41 12.9626071293692
42 12.9580332278612
43 12.9537370521356
44 12.9497261202601
45 12.9460080178853
46 12.9425902587191
47 12.9394801902069
48 12.9366849445411
49 12.9342114200891
50 12.9320662110573
51 12.9302553765358
52 12.9287840053962
53 12.9276556372011
54 12.9268717519043
55 12.9264315644258
56 12.926332289535
57 12.9263522615239
};
\addlegendentry{$J(\Omega)$}
\end{axis}

\end{tikzpicture}

